Generating Virtual On-body Accelerometer Data from Virtual Textual Descriptions for Human Activity Recognition

The development of robust, generalized models in human activity recognition (HAR) has been hindered by the scarcity of large-scale, labeled data sets. Recent work has shown that virtual IMU data extracted from videos using computer vision techniques can lead to substantial performance improvements when training HAR models combined with small portions of real IMU data. Inspired by recent advances in motion synthesis from textual descriptions and connecting Large Language Models (LLMs) to various AI models, we introduce an automated pipeline that first uses ChatGPT to generate diverse textual descriptions of activities. These textual descriptions are then used to generate 3D human motion sequences via a motion synthesis model, T2M-GPT, and later converted to streams of virtual IMU data. We benchmarked our approach on three HAR datasets (RealWorld, PAMAP2, and USC-HAD) and demonstrate that the use of virtual IMU training data generated using our new approach leads to significantly improved HAR model performance compared to only using real IMU data. Our approach contributes to the growing field of cross-modality transfer methods and illustrate how HAR models can be improved through the generation of virtual training data that do not require any manual effort.

==> sections/result/main.tex <==
\section{Result}
\thomas{We should not split 4 and 5. Make it one evaluation section. We also need experiments on more than one dataset.}
As shown in \autoref{tab:results}, the classifier trained on both real and virtual IMU data have improved performance compared to a classifier trained only real IMU data. The performance improvement is especially apparent when the reduced real IMU dataset is used. This shows the use of virtual IMU data for training is exceptionally beneficial when the amount of available real IMU data is limited.  

Furthermore, we observe that when data from all seven sensor locations are used, the classifier trained on only virtual IMU data outperforms the classifier trained on real IMU data. We find this surprising because the size of the virtual IMU dataset is less than 4\% of the size of the real IMU dataset. We attribute this performance imporvement to the diverse textual prompts that ChatGPT generated, which led to a diverse set of virtual IMU clips. Using such a diverse training data, the model learns to recognize the many variations of each activity. 

Overall, the two virtual IMU dataset led to classifiers with comparative performances with the exception of the classifier trained on only virtual IMU data from the forearm sensor. In this case, extracting joints' rotations by fitting the joints' positions to a SMPL model led to a better downstream classifier compared to using inverse kinematics for joints' rotations extraction. When inverse kinematics is used, the estimated rotations for joints farther in the kinematics chain will suffer from grater error due to error accumulation. Since the forearm joint is at the end of a kinematics chain, the error in the estimated forearm joint's rotations will be greater than that of the other joints, which leads to unrealistic virtual IMU data and in turn a worse classifier. However, we note that inverse kinematics is significantly faster than fitting to SMPL. On a RTX 2080ti, generating a five seconds clip of virtual IMU data takes five seconds using inverse kinematics, allowing real time generation, and one minute by fitting to SMPL.  





==> tables/f1_sensor.tex <==
 \begin{table}[t]
    \centering
    \vspace{-0.in}
    \caption{Model performances on the RealWorld dataset \cite{Sztyler2016realworld} for various scenerios. SMPL indicates the joints' rotations extracted by fitting joint positions to a SMPL model during virtual IMU data generation. IK indicates inverse kinematics is used during generation. The best performance within each scenario bolded. \thomas{2 digits after the decimal point are enough.} \zikang{I changed it to 3 digits to make sure that the confidence interval is not 0. }
    }
    \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular}{c|c|c|c|c}
          Sensors & Real Size & Dataset & F1  (SMPL) & F1 (IK) \\
         \hline\hline
         \multirow{6}{*}{Forearm} 
         & \multirow{3}{*}{110 minutes} & Real & $0.444 \pm 0.004$ &  $0.444 \pm 0.004$\\
         \cline{3-5}
         & & Virtual & $0.573 \pm 0.003$ & $0.523 \pm 0.003$ \\
         \cline{3-5}
         & & Real + Virtual & $0.589 \pm 0.005$ & $\textbf{0.602} \pm 0.012$\\
         \cline{3-5}
         \hhline{~====}
         & \multirow{3}{*}{1107 minutes} & Real & $0.613 \pm 0.006$ & $0.613 \pm 0.006$\\
         \cline{3-5}
         & & Virtual & $0.573 \pm 0.003$ & $0.523 \pm 0.003$  \\
         \cline{3-5}
         & & Real +Virtual & $\textbf{0.624} \pm 0.006$ & $0.620 \pm 0.002$ \\
         \cline{3-5}
         \hline\hline
         \multirow{6}{*}{All 7 sensors} 
          & \multirow{3}{*}{110 minutes} & Real & $0.481 \pm 0.009$ & $0.481 \pm 0.009$ \\
         \cline{3-5}
         & & Virtual & $0.752 \pm 0.003$ & $0.746 \pm 0.003$  \\
         \cline{3-5}
         & & Real + Virtual & $\textbf{0.776} \pm 0.008$ & $0.758 \pm 0.011$ \\
         \cline{3-5}
         \hhline{~====}
         & \multirow{3}{*}{1107 minutes} & Real & $0.715 \pm 0.011$ & $0.715 \pm 0.011$\\
         \cline{3-5}
         & & Virtual & $0.757 \pm 0.011$ & $0.746 \pm 0.003$  \\
         \cline{3-5}
         & & Real +Virtual & $0.769 \pm 0.004$ & $\textbf{0.770} \pm 0.004$ \\
         \cline{3-5}
         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:results}
    \vspace{-0.08in}
\end{table}

==> tables/f1_usc_had.tex <==
 \begin{table}[t]
    \centering
    \vspace{-0.in}
    \caption{Model performances on the USC-HAD \cite{Zhang2012usc} dataset. The best performance within each scenario bolded.
    }
    \begin{adjustbox}{width=0.6\columnwidth,center}
    \begin{tabular}{c|c|c}
          Real Size & Dataset & F1 Score \\
         \hline\hline
          \multirow{3}{*}{47 minutes} & Real 
         & $0.399 \pm 0.004$ \\
         \cline{2-3}
         & Virtual & $0.448 \pm 0.003$  \\
         \cline{2-3}
         & Real + Virtual & $\textbf{0.471} \pm 0.009$ \\
         \hline\hline
         \multirow{3}{*}{469 minutes} & Real 
         & $0.478 \pm 0.002$ \\
         \cline{2-3}
        &  Virtual & $0.448 \pm 0.003$  \\
         \cline{2-3}
         & Real +Virtual & $\textbf{0.486} \pm 0.003$  \\
         \cline{2-3}
         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:usc-had}
    \vspace{-0.08in}
\end{table}
